Code Copycat Conundrum: Demystifying Repetition in LLM-based Code Generation

Despite recent advances in Large Language Models (LLMs) for code generation, the quality of LLM-generated code still faces significant challenges. One significant issue is code repetition, which refers to the model's tendency to generate structurally redundant code, resulting in inefficiencies and reduced readability. To address this, we conduct the first empirical study to investigate the prevalence and nature of repetition across 19 state-of-the-art code LLMs using three widely-used benchmarks. Our study includes both quantitative and qualitative analyses, revealing that repetition is pervasive and manifests at various granularities and extents, including character, statement, and block levels. We further summarize a taxonomy of 20 repetition patterns. Building on our findings, we propose DeRep, a rule-based technique designed to detect and mitigate repetition in generated code. We evaluate DeRep using both open-source benchmarks and in an industrial setting. Our results demonstrate that DeRep significantly outperforms baselines in reducing repetition (with an average improvements of 91.3%, 93.5%, and 79.9% in rep-3, rep-line, and sim-line metrics) and enhancing code quality (with a Pass@1 increase of 208.3% over greedy search). Furthermore, integrating DeRep improves the performance of existing repetition mitigation methods, with Pass@1 improvements ranging from 53.7% to 215.7%.

==> algorithm/repair.tex <==
\begin{algorithm}[ht]
\caption{Repetition Repair Algorithm}
\label{alg:fix_repeats}
\begin{algorithmic}[1]
\Require $code$
\Ensure $fixedCode$
\State $lines \gets \text{array of lines in } code$
\State $n \gets \text{length}(lines)$
\State $extraLines \gets \text{array of size } n \text{ initialized to false}$
\For{$blockSize \gets 1$ to $\left\lfloor \frac{n}{2} \right\rfloor$}
    \State $isRepeated \gets \text{array of size } n \text{ initialized to false}$
    \For{$i \gets 0$ to $n - 2 \times blockSize$}
        \If{$lines[i:i+blockSize] \approx lines[i+blockSize:i+2 \times blockSize]$}
            \State $isRepeated[i+blockSize:i+2 \times blockSize] \gets \text{true}$
        \EndIf
    \EndFor
    \For{$item$ in parts of consecutive trues in $isRepeated$}
        \If{length$(item)$ exceeds expected value}
            \State $s, e \gets \text{start and end of } item$
            \State $extraLines[s + blocksize:e] \gets \text{true}$
        \EndIf
    \EndFor
    
\EndFor
\State Initialize $fixedLines \gets \text{empty list}$
\For{$i \gets 0$ to $n-1$}
    \If{$extraLines[i] = \text{false}$}
        \State Append $lines[i]$ to $fixedLines$
    \EndIf
\EndFor
\Return \text{Join all elements of } $fixedLines$ \text{ into a single code string}
\end{algorithmic}
\end{algorithm}


==> tables/metrics2.tex <==
\begin{table}[]
\centering
\caption{Performance Comparison of Repetition Mitigation Techniques: Pre- (Red) and Post- (Green) Application of DeRep (CT: Contrastive Search)}
\label{tab-rq3}
\scriptsize
\setlength{\tabcolsep}{0pt}
\begin{tabular}{|lllllll|}
\hline
\multicolumn{1}{|l|}{}           & \multicolumn{1}{c|}{Greedy}                                                & \multicolumn{1}{c|}{Beam(3)}                                               & \multicolumn{1}{c|}{Top-k(10)}                                             & \multicolumn{1}{c|}{Top-p(0.85)}                                           & \multicolumn{1}{c|}{CT(0.6)}                                               & Penalty(1.2)                                          \\ \hline
\multicolumn{7}{|c|}{rep-3}                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b}   & \multicolumn{1}{l|}{\textcolor{red}{45.1}->\textcolor[rgb]{0,0.5,0}{5.2}}  & \multicolumn{1}{l|}{\textcolor{red}{29.1}->\textcolor[rgb]{0,0.5,0}{5.8}}  & \multicolumn{1}{l|}{\textcolor{red}{9.1}->\textcolor[rgb]{0,0.5,0}{5.3}}   & \multicolumn{1}{l|}{\textcolor{red}{11.5}->\textcolor[rgb]{0,0.5,0}{4.3}}  & \multicolumn{1}{l|}{\textcolor{red}{1.8}->\textcolor[rgb]{0,0.5,0}{1.7}}   & \textcolor{red}{1.4}->\textcolor[rgb]{0,0.5,0}{1.2}   \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b-I} & \multicolumn{1}{l|}{\textcolor{red}{37.6}->\textcolor[rgb]{0,0.5,0}{4.0}}  & \multicolumn{1}{l|}{\textcolor{red}{31.2}->\textcolor[rgb]{0,0.5,0}{3.7}}  & \multicolumn{1}{l|}{\textcolor{red}{17.2}->\textcolor[rgb]{0,0.5,0}{4.0}}  & \multicolumn{1}{l|}{\textcolor{red}{23.6}->\textcolor[rgb]{0,0.5,0}{4.2}}  & \multicolumn{1}{l|}{\textcolor{red}{23.5}->\textcolor[rgb]{0,0.5,0}{3.8}}  & \textcolor{red}{0.1}->\textcolor[rgb]{0,0.5,0}{0.0}   \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b}   & \multicolumn{1}{l|}{\textcolor{red}{43.6}->\textcolor[rgb]{0,0.5,0}{4.3}}  & \multicolumn{1}{l|}{\textcolor{red}{29.6}->\textcolor[rgb]{0,0.5,0}{5.1}}  & \multicolumn{1}{l|}{\textcolor{red}{7.7}->\textcolor[rgb]{0,0.5,0}{4.0}}   & \multicolumn{1}{l|}{\textcolor{red}{10.5}->\textcolor[rgb]{0,0.5,0}{4.4}}  & \multicolumn{1}{l|}{\textcolor{red}{3.3}->\textcolor[rgb]{0,0.5,0}{2.8}}   & \textcolor{red}{2.1}->\textcolor[rgb]{0,0.5,0}{1.8}   \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b-I} & \multicolumn{1}{l|}{\textcolor{red}{37.2}->\textcolor[rgb]{0,0.5,0}{2.5}}  & \multicolumn{1}{l|}{\textcolor{red}{32.0}->\textcolor[rgb]{0,0.5,0}{3.1}}  & \multicolumn{1}{l|}{\textcolor{red}{15.0}->\textcolor[rgb]{0,0.5,0}{3.0}}  & \multicolumn{1}{l|}{\textcolor{red}{19.2}->\textcolor[rgb]{0,0.5,0}{3.2}}  & \multicolumn{1}{l|}{\textcolor{red}{12.9}->\textcolor[rgb]{0,0.5,0}{2.7}}  & \textcolor{red}{4.2}->\textcolor[rgb]{0,0.5,0}{1.8}   \\ \hline
\multicolumn{1}{|l|}{DSC-33b}    & \multicolumn{1}{l|}{\textcolor{red}{38.2}->\textcolor[rgb]{0,0.5,0}{3.2}}  & \multicolumn{1}{l|}{\textcolor{red}{24.3}->\textcolor[rgb]{0,0.5,0}{3.2}}  & \multicolumn{1}{l|}{\textcolor{red}{8.5}->\textcolor[rgb]{0,0.5,0}{3.2}}   & \multicolumn{1}{l|}{\textcolor{red}{15.1}->\textcolor[rgb]{0,0.5,0}{3.3}}  & \multicolumn{1}{l|}{\textcolor{red}{5.9}->\textcolor[rgb]{0,0.5,0}{2.0}}   & \textcolor{red}{2.5}->\textcolor[rgb]{0,0.5,0}{2.0}   \\ \hline
\multicolumn{1}{|l|}{DSC-33b-I}  & \multicolumn{1}{l|}{\textcolor{red}{39.2}->\textcolor[rgb]{0,0.5,0}{2.0}}  & \multicolumn{1}{l|}{\textcolor{red}{35.6}->\textcolor[rgb]{0,0.5,0}{3.2}}  & \multicolumn{1}{l|}{\textcolor{red}{10.1}->\textcolor[rgb]{0,0.5,0}{2.7}}  & \multicolumn{1}{l|}{\textcolor{red}{18.0}->\textcolor[rgb]{0,0.5,0}{2.2}}  & \multicolumn{1}{l|}{\textcolor{red}{11.1}->\textcolor[rgb]{0,0.5,0}{2.1}}  & \textcolor{red}{6.2}->\textcolor[rgb]{0,0.5,0}{3.0}   \\ \hline
\multicolumn{1}{|l|}{Average}    & \multicolumn{1}{l|}{\textcolor{red}{40.2}->\textcolor[rgb]{0,0.5,0}{3.5}}  & \multicolumn{1}{l|}{\textcolor{red}{30.3}->\textcolor[rgb]{0,0.5,0}{4.0}}  & \multicolumn{1}{l|}{\textcolor{red}{11.3}->\textcolor[rgb]{0,0.5,0}{3.7}}  & \multicolumn{1}{l|}{\textcolor{red}{16.3}->\textcolor[rgb]{0,0.5,0}{3.6}}  & \multicolumn{1}{l|}{\textcolor{red}{9.8}->\textcolor[rgb]{0,0.5,0}{2.5}}   & \textcolor{red}{2.8}->\textcolor[rgb]{0,0.5,0}{1.6}   \\ \hline
\multicolumn{1}{|l|}{Pre-DeRep}  & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-24.6\%}                                               & \multicolumn{1}{c|}{-71.9\%}                                               & \multicolumn{1}{c|}{-59.5\%}                                               & \multicolumn{1}{c|}{-75.6\%}                                               & \multicolumn{1}{c|}{\textbf{-93.0\%}}                 \\ \hline
\multicolumn{1}{|l|}{Post-DeRep} & \multicolumn{1}{c|}{-91.3\%}                                               & \multicolumn{1}{c|}{-90.0\%}                                               & \multicolumn{1}{c|}{-90.8\%}                                               & \multicolumn{1}{c|}{-91.0\%}                                               & \multicolumn{1}{c|}{-93.8\%}                                               & \multicolumn{1}{c|}{\textbf{-96.0\%}}                 \\ \hline
\multicolumn{7}{|c|}{rep-line}                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b}   & \multicolumn{1}{l|}{\textcolor{red}{28.4}->\textcolor[rgb]{0,0.5,0}{2.1}}  & \multicolumn{1}{l|}{\textcolor{red}{16.7}->\textcolor[rgb]{0,0.5,0}{2.7}}  & \multicolumn{1}{l|}{\textcolor{red}{4.5}->\textcolor[rgb]{0,0.5,0}{1.9}}   & \multicolumn{1}{l|}{\textcolor{red}{6.4}->\textcolor[rgb]{0,0.5,0}{1.6}}   & \multicolumn{1}{l|}{\textcolor{red}{0.4}->\textcolor[rgb]{0,0.5,0}{0.4}}   & \textcolor{red}{0.0}->\textcolor[rgb]{0,0.5,0}{0.1}   \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b-I} & \multicolumn{1}{l|}{\textcolor{red}{18.5}->\textcolor[rgb]{0,0.5,0}{1.0}}  & \multicolumn{1}{l|}{\textcolor{red}{16.8}->\textcolor[rgb]{0,0.5,0}{1.1}}  & \multicolumn{1}{l|}{\textcolor{red}{13.0}->\textcolor[rgb]{0,0.5,0}{1.4}}  & \multicolumn{1}{l|}{\textcolor{red}{10.1}->\textcolor[rgb]{0,0.5,0}{1.0}}  & \multicolumn{1}{l|}{\textcolor{red}{8.1}->\textcolor[rgb]{0,0.5,0}{1.0}}   & \textcolor{red}{0.0}->\textcolor[rgb]{0,0.5,0}{0.0}   \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b}   & \multicolumn{1}{l|}{\textcolor{red}{30.5}->\textcolor[rgb]{0,0.5,0}{1.9}}  & \multicolumn{1}{l|}{\textcolor{red}{17.0}->\textcolor[rgb]{0,0.5,0}{2.1}}  & \multicolumn{1}{l|}{\textcolor{red}{4.3}->\textcolor[rgb]{0,0.5,0}{1.3}}   & \multicolumn{1}{l|}{\textcolor{red}{5.6}->\textcolor[rgb]{0,0.5,0}{1.7}}   & \multicolumn{1}{l|}{\textcolor{red}{0.9}->\textcolor[rgb]{0,0.5,0}{0.8}}   & \textcolor{red}{0.4}->\textcolor[rgb]{0,0.5,0}{0.4}   \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b-I} & \multicolumn{1}{l|}{\textcolor{red}{23.8}->\textcolor[rgb]{0,0.5,0}{1.1}}  & \multicolumn{1}{l|}{\textcolor{red}{21.3}->\textcolor[rgb]{0,0.5,0}{1.1}}  & \multicolumn{1}{l|}{\textcolor{red}{11.4}->\textcolor[rgb]{0,0.5,0}{0.9}}  & \multicolumn{1}{l|}{\textcolor{red}{13.0}->\textcolor[rgb]{0,0.5,0}{1.3}}  & \multicolumn{1}{l|}{\textcolor{red}{7.7}->\textcolor[rgb]{0,0.5,0}{1.0}}   & \textcolor{red}{1.6}->\textcolor[rgb]{0,0.5,0}{0.7}   \\ \hline
\multicolumn{1}{|l|}{DSC-33b}    & \multicolumn{1}{l|}{\textcolor{red}{20.3}->\textcolor[rgb]{0,0.5,0}{1.1}}  & \multicolumn{1}{l|}{\textcolor{red}{11.7}->\textcolor[rgb]{0,0.5,0}{1.3}}  & \multicolumn{1}{l|}{\textcolor{red}{4.4}->\textcolor[rgb]{0,0.5,0}{1.0}}   & \multicolumn{1}{l|}{\textcolor{red}{7.5}->\textcolor[rgb]{0,0.5,0}{1.4}}   & \multicolumn{1}{l|}{\textcolor{red}{2.8}->\textcolor[rgb]{0,0.5,0}{0.9}}   & \textcolor{red}{0.6}->\textcolor[rgb]{0,0.5,0}{0.5}   \\ \hline
\multicolumn{1}{|l|}{DSC-33b-I}  & \multicolumn{1}{l|}{\textcolor{red}{16.6}->\textcolor[rgb]{0,0.5,0}{1.0}}  & \multicolumn{1}{l|}{\textcolor{red}{16.2}->\textcolor[rgb]{0,0.5,0}{1.2}}  & \multicolumn{1}{l|}{\textcolor{red}{5.7}->\textcolor[rgb]{0,0.5,0}{1.0}}   & \multicolumn{1}{l|}{\textcolor{red}{8.1}->\textcolor[rgb]{0,0.5,0}{1.0}}   & \multicolumn{1}{l|}{\textcolor{red}{5.1}->\textcolor[rgb]{0,0.5,0}{0.8}}   & \textcolor{red}{2.2}->\textcolor[rgb]{0,0.5,0}{1.2}   \\ \hline
\multicolumn{1}{|l|}{Average}    & \multicolumn{1}{l|}{\textcolor{red}{23.0}->\textcolor[rgb]{0,0.5,0}{1.5}}  & \multicolumn{1}{l|}{\textcolor{red}{16.6}->\textcolor[rgb]{0,0.5,0}{1.6}}  & \multicolumn{1}{l|}{\textcolor{red}{7.2}->\textcolor[rgb]{0,0.5,0}{1.2}}   & \multicolumn{1}{l|}{\textcolor{red}{8.5}->\textcolor[rgb]{0,0.5,0}{1.3}}   & \multicolumn{1}{l|}{\textcolor{red}{4.2}->\textcolor[rgb]{0,0.5,0}{0.8}}   & \textcolor{red}{0.8}->\textcolor[rgb]{0,0.5,0}{0.5}   \\ \hline
\multicolumn{1}{|l|}{Pre-DeRep}  & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-27.8\%}                                               & \multicolumn{1}{c|}{-68.7\%}                                               & \multicolumn{1}{c|}{-63.0\%}                                               & \multicolumn{1}{c|}{-81.7\%}                                               & \multicolumn{1}{c|}{\textbf{-96.5\%}}                 \\ \hline
\multicolumn{1}{|l|}{Post-DeRep} & \multicolumn{1}{c|}{-93.5\%}                                               & \multicolumn{1}{c|}{-93.0\%}                                               & \multicolumn{1}{c|}{-94.8\%}                                               & \multicolumn{1}{c|}{-94.3\%}                                               & \multicolumn{1}{c|}{-96.5\%}                                               & \multicolumn{1}{c|}{\textbf{-97.8\%}}                 \\ \hline
\multicolumn{7}{|c|}{sim-line}                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b}   & \multicolumn{1}{l|}{\textcolor{red}{31.1}->\textcolor[rgb]{0,0.5,0}{6.8}}  & \multicolumn{1}{l|}{\textcolor{red}{20.0}->\textcolor[rgb]{0,0.5,0}{6.4}}  & \multicolumn{1}{l|}{\textcolor{red}{4.2}->\textcolor[rgb]{0,0.5,0}{3.7}}   & \multicolumn{1}{l|}{\textcolor{red}{8.8}->\textcolor[rgb]{0,0.5,0}{4.0}}   & \multicolumn{1}{l|}{\textcolor{red}{1.2}->\textcolor[rgb]{0,0.5,0}{1.1}}   & \textcolor{red}{0.5}->\textcolor[rgb]{0,0.5,0}{0.4}   \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b-I} & \multicolumn{1}{l|}{\textcolor{red}{31.1}->\textcolor[rgb]{0,0.5,0}{6.0}}  & \multicolumn{1}{l|}{\textcolor{red}{28.1}->\textcolor[rgb]{0,0.5,0}{5.8}}  & \multicolumn{1}{l|}{\textcolor{red}{9.4}->\textcolor[rgb]{0,0.5,0}{5.5}}   & \multicolumn{1}{l|}{\textcolor{red}{18.2}->\textcolor[rgb]{0,0.5,0}{5.6}}  & \multicolumn{1}{l|}{\textcolor{red}{14.2}->\textcolor[rgb]{0,0.5,0}{4.9}}  & \textcolor{red}{1.4}->\textcolor[rgb]{0,0.5,0}{1.1}   \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b}   & \multicolumn{1}{l|}{\textcolor{red}{35.3}->\textcolor[rgb]{0,0.5,0}{7.1}}  & \multicolumn{1}{l|}{\textcolor{red}{23.0}->\textcolor[rgb]{0,0.5,0}{6.8}}  & \multicolumn{1}{l|}{\textcolor{red}{6.0}->\textcolor[rgb]{0,0.5,0}{4.4}}   & \multicolumn{1}{l|}{\textcolor{red}{10.3}->\textcolor[rgb]{0,0.5,0}{4.6}}  & \multicolumn{1}{l|}{\textcolor{red}{2.6}->\textcolor[rgb]{0,0.5,0}{1.9}}   & \textcolor{red}{0.6}->\textcolor[rgb]{0,0.5,0}{0.6}   \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b-I} & \multicolumn{1}{l|}{\textcolor{red}{32.2}->\textcolor[rgb]{0,0.5,0}{5.7}}  & \multicolumn{1}{l|}{\textcolor{red}{28.3}->\textcolor[rgb]{0,0.5,0}{6.6}}  & \multicolumn{1}{l|}{\textcolor{red}{11.8}->\textcolor[rgb]{0,0.5,0}{5.3}}  & \multicolumn{1}{l|}{\textcolor{red}{16.2}->\textcolor[rgb]{0,0.5,0}{6.0}}  & \multicolumn{1}{l|}{\textcolor{red}{13.5}->\textcolor[rgb]{0,0.5,0}{5.2}}  & \textcolor{red}{4.4}->\textcolor[rgb]{0,0.5,0}{2.5}   \\ \hline
\multicolumn{1}{|l|}{DSC-33b}    & \multicolumn{1}{l|}{\textcolor{red}{22.5}->\textcolor[rgb]{0,0.5,0}{4.8}}  & \multicolumn{1}{l|}{\textcolor{red}{11.7}->\textcolor[rgb]{0,0.5,0}{4.0}}  & \multicolumn{1}{l|}{\textcolor{red}{4.4}->\textcolor[rgb]{0,0.5,0}{2.9}}   & \multicolumn{1}{l|}{\textcolor{red}{7.5}->\textcolor[rgb]{0,0.5,0}{4.4}}   & \multicolumn{1}{l|}{\textcolor{red}{2.8}->\textcolor[rgb]{0,0.5,0}{2.2}}   & \textcolor{red}{0.6}->\textcolor[rgb]{0,0.5,0}{0.5}   \\ \hline
\multicolumn{1}{|l|}{DSC-33b-I}  & \multicolumn{1}{l|}{\textcolor{red}{21.8}->\textcolor[rgb]{0,0.5,0}{4.6}}  & \multicolumn{1}{l|}{\textcolor{red}{18.2}->\textcolor[rgb]{0,0.5,0}{5.1}}  & \multicolumn{1}{l|}{\textcolor{red}{5.4}->\textcolor[rgb]{0,0.5,0}{3.1}}   & \multicolumn{1}{l|}{\textcolor{red}{7.8}->\textcolor[rgb]{0,0.5,0}{3.9}}   & \multicolumn{1}{l|}{\textcolor{red}{2.4}->\textcolor[rgb]{0,0.5,0}{1.9}}   & \textcolor{red}{0.9}->\textcolor[rgb]{0,0.5,0}{0.7}   \\ \hline
\multicolumn{1}{|l|}{Average}    & \multicolumn{1}{l|}{\textcolor{red}{28.9}->\textcolor[rgb]{0,0.5,0}{5.8}}  & \multicolumn{1}{l|}{\textcolor{red}{21.6}->\textcolor[rgb]{0,0.5,0}{5.8}}  & \multicolumn{1}{l|}{\textcolor{red}{6.9}->\textcolor[rgb]{0,0.5,0}{4.2}}   & \multicolumn{1}{l|}{\textcolor{red}{11.5}->\textcolor[rgb]{0,0.5,0}{4.8}}  & \multicolumn{1}{l|}{\textcolor{red}{6.1}->\textcolor[rgb]{0,0.5,0}{2.9}}   & \textcolor{red}{1.4}->\textcolor[rgb]{0,0.5,0}{1.0}   \\ \hline
\multicolumn{1}{|l|}{Pre-DeRep}  & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-25.3\%}                                               & \multicolumn{1}{c|}{-76.1\%}                                               & \multicolumn{1}{c|}{-60.2\%}                                               & \multicolumn{1}{c|}{-78.9\%}                                               & \multicolumn{1}{c|}{\textbf{-95.2\%}}                 \\ \hline
\multicolumn{1}{|l|}{Post-DeRep} & \multicolumn{1}{c|}{-79.9\%}                                               & \multicolumn{1}{c|}{-79.9\%}                                               & \multicolumn{1}{c|}{-85.5\%}                                               & \multicolumn{1}{c|}{-83.4\%}                                               & \multicolumn{1}{c|}{-90.0\%}                                               & \multicolumn{1}{c|}{\textbf{-96.5\%}}                 \\ \hline
\multicolumn{7}{|c|}{Pass@1}                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b}   & \multicolumn{1}{l|}{\textcolor{red}{2.9}->\textcolor[rgb]{0,0.5,0}{22.6}}  & \multicolumn{1}{l|}{\textcolor{red}{11.0}->\textcolor[rgb]{0,0.5,0}{23.5}} & \multicolumn{1}{l|}{\textcolor{red}{13.2}->\textcolor[rgb]{0,0.5,0}{13.2}} & \multicolumn{1}{l|}{\textcolor{red}{11.3}->\textcolor[rgb]{0,0.5,0}{16.1}} & \multicolumn{1}{l|}{\textcolor{red}{11.0}->\textcolor[rgb]{0,0.5,0}{11.3}} & \textcolor{red}{7.7}->\textcolor[rgb]{0,0.5,0}{7.7}   \\ \hline
\multicolumn{1}{|l|}{DSC-1.3b-I} & \multicolumn{1}{l|}{\textcolor{red}{18.5}->\textcolor[rgb]{0,0.5,0}{40.4}} & \multicolumn{1}{l|}{\textcolor{red}{9.4}->\textcolor[rgb]{0,0.5,0}{38.1}}  & \multicolumn{1}{l|}{\textcolor{red}{12.9}->\textcolor[rgb]{0,0.5,0}{31.4}} & \multicolumn{1}{l|}{\textcolor{red}{7.6}->\textcolor[rgb]{0,0.5,0}{33.6}}  & \multicolumn{1}{l|}{\textcolor{red}{8.1}->\textcolor[rgb]{0,0.5,0}{28.4}}  & \textcolor{red}{0.2}->\textcolor[rgb]{0,0.5,0}{0.4}   \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b}   & \multicolumn{1}{l|}{\textcolor{red}{5.7}->\textcolor[rgb]{0,0.5,0}{24.9}}  & \multicolumn{1}{l|}{\textcolor{red}{17.7}->\textcolor[rgb]{0,0.5,0}{27.5}} & \multicolumn{1}{l|}{\textcolor{red}{15.5}->\textcolor[rgb]{0,0.5,0}{16.4}} & \multicolumn{1}{l|}{\textcolor{red}{12.8}->\textcolor[rgb]{0,0.5,0}{20.8}} & \multicolumn{1}{l|}{\textcolor{red}{17.7}->\textcolor[rgb]{0,0.5,0}{17.3}} & \textcolor{red}{10.6}->\textcolor[rgb]{0,0.5,0}{11.1} \\ \hline
\multicolumn{1}{|l|}{DSC-6.7b-I} & \multicolumn{1}{l|}{\textcolor{red}{8.2}->\textcolor[rgb]{0,0.5,0}{43.5}}  & \multicolumn{1}{l|}{\textcolor{red}{8.2}->\textcolor[rgb]{0,0.5,0}{44.7}}  & \multicolumn{1}{l|}{\textcolor{red}{12.1}->\textcolor[rgb]{0,0.5,0}{38.8}} & \multicolumn{1}{l|}{\textcolor{red}{9.5}->\textcolor[rgb]{0,0.5,0}{42.6}}  & \multicolumn{1}{l|}{\textcolor{red}{23.1}->\textcolor[rgb]{0,0.5,0}{40.0}} & \textcolor{red}{17.0}->\textcolor[rgb]{0,0.5,0}{26.3} \\ \hline
\multicolumn{1}{|l|}{DSC-33b}    & \multicolumn{1}{l|}{\textcolor{red}{14.4}->\textcolor[rgb]{0,0.5,0}{30.0}} & \multicolumn{1}{l|}{\textcolor{red}{19.3}->\textcolor[rgb]{0,0.5,0}{28.5}} & \multicolumn{1}{l|}{\textcolor{red}{14.0}->\textcolor[rgb]{0,0.5,0}{21.2}} & \multicolumn{1}{l|}{\textcolor{red}{16.9}->\textcolor[rgb]{0,0.5,0}{22.7}} & \multicolumn{1}{l|}{\textcolor{red}{21.2}->\textcolor[rgb]{0,0.5,0}{26.5}} & \textcolor{red}{22.7}->\textcolor[rgb]{0,0.5,0}{22.2} \\ \hline
\multicolumn{1}{|l|}{DSC-33b-I}  & \multicolumn{1}{l|}{\textcolor{red}{15.3}->\textcolor[rgb]{0,0.5,0}{38.5}} & \multicolumn{1}{l|}{\textcolor{red}{24.8}->\textcolor[rgb]{0,0.5,0}{42.0}} & \multicolumn{1}{l|}{\textcolor{red}{22.4}->\textcolor[rgb]{0,0.5,0}{27.8}} & \multicolumn{1}{l|}{\textcolor{red}{18.0}->\textcolor[rgb]{0,0.5,0}{34.9}} & \multicolumn{1}{l|}{\textcolor{red}{29.5}->\textcolor[rgb]{0,0.5,0}{34.3}} & \textcolor{red}{31.3}->\textcolor[rgb]{0,0.5,0}{31.9} \\ \hline
\multicolumn{1}{|l|}{Average}    & \multicolumn{1}{l|}{\textcolor{red}{10.8}->\textcolor[rgb]{0,0.5,0}{33.3}} & \multicolumn{1}{l|}{\textcolor{red}{15.1}->\textcolor[rgb]{0,0.5,0}{34.1}} & \multicolumn{1}{l|}{\textcolor{red}{15.0}->\textcolor[rgb]{0,0.5,0}{24.8}} & \multicolumn{1}{l|}{\textcolor{red}{12.7}->\textcolor[rgb]{0,0.5,0}{28.5}} & \multicolumn{1}{l|}{\textcolor{red}{18.4}->\textcolor[rgb]{0,0.5,0}{26.3}} & \textcolor{red}{14.9}->\textcolor[rgb]{0,0.5,0}{16.6} \\ \hline
\multicolumn{1}{|l|}{Pre-DeRep}  & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{+39.8\%}                                               & \multicolumn{1}{c|}{+38.9\%}                                               & \multicolumn{1}{c|}{+17.6\%}                                               & \multicolumn{1}{c|}{\textbf{+70.4\%}}                                      & \multicolumn{1}{c|}{+38.0\%}                          \\ \hline
\multicolumn{1}{|l|}{Post-DeRep} & \multicolumn{1}{c|}{+208.3\%}                                              & \multicolumn{1}{c|}{\textbf{+215.7\%}}                                     & \multicolumn{1}{c|}{+129.6\%}                                              & \multicolumn{1}{c|}{+163.9\%}                                              & \multicolumn{1}{c|}{+143.5\%}                                              & \multicolumn{1}{c|}{+53.7\%}                          \\ \hline
\end{tabular}
\end{table}
